QDB: From Quantum Algorithms Towards Correct Quantum Programs

With the advent of small-scale prototype quantum computers, researchers can now code and run quantum algorithms that were previously proposed but not fully implemented. In support of this growing interest in quantum computing experimentation, programmers need new tools and techniques to write and debug QC code. In this work, we implement a range of QC algorithms and programs in order to discover what types of bugs occur and what defenses against those bugs are possible in QC programs. We conduct our study by running small-sized QC programs in QC simulators in order to replicate published results in QC implementations. Where possible, we cross-validate results from programs written in different QC languages for the same problems and inputs. Drawing on this experience, we provide a taxonomy for QC bugs, and we propose QC language features that would aid in writing correct code.

==> _bug_taxonomy.tex <==
\section{QC programming and runtime bugs}


\begin{table*}
\caption{Taxonomy of quantum program bugs, following example of classical programming bugs in Ref.~\cite{Altadmri}}
\centering
\begin{tabularx}{\linewidth}{ |p{2cm}|l|X| }
\hline
\textbf{Bug type} & \textbf{Algorithm} & \textbf{Bug description} \\
\hline
\hline

\multirow{3}{2cm}{Mistake in classical input parameters} & Hamiltonian simulation & Wrong classical parameters for molecular integrals \\\cline{2-3}
& Shor's factorization & Wrong input powers of numbers in modular basis \\\cline{2-3}
& Grover's search & Wrong assumption on number of matches in database \\\hline
Wrong initial values & Hamiltonian simulation & Simulation of the wrong molecular energy state because of incorrect input eigenstate \\\hline

\multirow{4}{2cm}{Wrong operation or transformation} & Hamiltonian simulation & Mistake changing basis between Pauli X, Y, Z bases \\\cline{2-3}
& QFT & Confusion of phase shifts and rotations \\\cline{2-3}
& QFT & Confusion of CNOT control and target \\\cline{2-3}
& Grover's search & Bad oracle construction for classical property check \\\hline

\multirow{2}{2cm}{Wrong indexing} & QFT & Mistake in Fourier transform recursion/iteration code \\\cline{2-3}
& Shor's factorization & Qubit indexing error in overflow/carry bits \\\hline

\multirow{2}{2cm}{Wrong numeric encoding} & QFT & Confusion whether to reverse output qubits order \\\cline{2-3}
& Shor's factorization & Mistaking most/least significant bits in phase estimation \\\hline

Improper deallocation of ancillary qubits & Shor's factorization & Improperly mirrored operations for reversible computation \\\hline

\multirow{3}{2cm}{Failure of algorithm progress} & Hamiltonian simulation & Insufficient number of Trotter steps \\\cline{2-3}
& Shor's factorization & Insufficient number of phase estimation iterations \\\cline{2-3}
& Grover's search & Incorrect number of iterations \\\hline

\end{tabularx}
\label{tab:bug_taxonomy}
\end{table*}

We list categories of bugs and their examples in different QC algorithms in Table~\ref{tab:bug_taxonomy}.
% One defense would be to use formal verification to make sure QC programs match QC algorithm specifications~\cite{quipper,quipper_cacm}.
% This paper explores how language features and pragmatic techniques like cross-validation can also eliminate these types of bugs.

% On the other hand, correctly specified quantum programs can still give wrong results due to qubit corruption, unreliable operations, and errors in measurement.
% These types of errors are handled via quantum error correction codes~\cite{quantum_error_correction}.
% Error correction techniques are costly in terms of number of qubits and operations, so they are likely impractical in the near term~\cite{Preskill2018computinginnisqera}.
% This paper explores how lightweight checks such as assertions can nonetheless catch some runtime bugs.


% % It's also possible that a program is correct, but errors occur during its execution due to decay of the state of qubits or faulty measurement.
% % Those important concerns are addressed via quantum error correction~\cite{quantum_error_correction} and language support for runtime assertions (Section~\ref{sec:assertions}).

==> _simulation.tex <==
\subsection{Combination of emulation and stabilizer simulation}
\label{sec:simulation}
A final benefit of writing modular quantum programs is it helps with efficiently simulating quantum programs in a classical computer,
which in turn enables us to debug larger quantum programs in simulation.
Specifically, it allows a future approach that combines two important and complementary ideas in quantum program simulation:
\begin{enumerate*}
\item emulation of program behavior,
\item efficient simulation of stabilizer circuits.
\end{enumerate*}

\emph{Emulation} is a simulation technique that replaces blocks of quantum programs with their behavioral equivalent~\cite{emulation}.
For example, a QFT subroutine would compile to a behavioral model using fast Fourier transform for simulation,
which would be more efficient than simulating the fully decomposed quantum gates that comprise QFT.
A potential downside of emulation is it works for a limited set of quantum program kernels that do have behavioral models,
such as QFT, adders, multipliers, and black-box oracles.

In contrast, \emph{stabilizer circuits} are an efficient simulation technique that doesn't care about quantum program behavior;
instead, it is able to efficiently simulate any part of the program that uses a non-universal subset of quantum gates called the Clifford gates~\cite{simulation_stabilizer}.
In many quantum algorithms, the non-Clifford gates that would prevent efficient stabilizer simulation show up only in specific subroutines.
Language syntax support for reversible computation and controlled operations (Section~\ref{sec:syntax}) helps cut down on these problematic gates.
In our case studies as examples:
\begin{itemize}
\item In quantum chemistry applications, non-Clifford gates are local to the rotations in subroutines for finding the Hamiltonian.
\item In Shor's factorization algorithm, the non-Clifford gates are local to two subroutines: in Toffoli gates for controlled-swap gates, and in rotations on Fourier-space data.
\item In Grover's search algorithm, the non-Clifford gates are local to Toffoli gates for controlled operations, and possibly in the oracle.
\end{itemize}

In a combined simulation strategy, one could use emulation to behaviorally model subroutines with many non-Clifford gates, reducing the penalty of having to simulate non-Clifford gates in stabilizer simulators.

% Clifford set is integer
% Non-clifford set is real
% Microsoft Clifford-only simulator
% CHP open source Clifford only simulator
